Improving Self-supervised Molecular Representation Learning using Persistent Homology

Self-supervised learning (SSL) has great potential for molecular representation learning given the complexity of molecular graphs, the large amounts of unlabelled data available, the considerable cost of obtaining labels experimentally, and the hence often only small training datasets. The importance of the topic is reflected in the variety of paradigms and architectures that have been investigated recently. Yet the differences in performance seem often minor and are barely understood to date. In this paper, we study SSL based on persistent homology (PH), a mathematical tool for modeling topological features of data that persist across multiple scales. It has several unique features which particularly suit SSL, naturally offering: different views of the data, stability in terms of distance preservation, and the opportunity to flexibly incorporate domain knowledge. We (1) investigate an autoencoder, which shows the general representational power of PH, and (2) propose a contrastive loss that complements existing approaches. We rigorously evaluate our approach for molecular property prediction and demonstrate its particular features in improving the embedding space: after SSL, the representations are better and offer considerably more predictive power than the baselines over different probing tasks; our loss increases baseline performance, sometimes largely; and we often obtain substantial improvements over very small datasets, a common scenario in practice.

==> intro.tex <==

\newpage
needed in end
\begin{itemize}
\item rogi, refs
\item sega update if icml reference
\item need to explain something for GEOM?
\item structure appendix to have correct tab fig numbers in paper
 \item think what to write about all other experniments eg regresison
\item check: do all tables contain all baselines?
    \item fix figure style, also make same in all
    \item neurips additional files, broader impact.., code
    \item table coloring
   \item most recent papers, icml..
   \item discuss how to add other models, 3 best/recent on zinc 15? 3 best CL ? ...
   \item mention in appendix filtration switch, GIN..
   \item LATER distance to seen previously, train spec or include in training
\end{itemize}

Evaluation Plan 
The gray parts mention additional information or things we should keep in mind as not critical but impactful/great to have.
\begin{enumerate}

% \item Some intro analysis about advantages of homology SSL

% I PIs offer a useful embedding space - shown in  the pic we had on slack on April 2nd showing the cosine similarities match the molecule similarity; Fig \ref{fig:pi-space-uselful-fp-sim}

% I [L] Homology Pre-training is successful/feasible: 

% 1 PIP successfully produces PIs on FT data,  Table \ref{tab:PI-pearson} %and hopefully is calibrated on that data 
% %(similar to earlier \#E2) \tbd{where is this shown, don't remember right now. in Tab 1, the MSE seems too large? or do you think it is OK} \luo{Table \ref{tab:PI-pearson} explains this. It should be that PIP successfully produces PIs for downstream tasks. It is obvious that PIP successfully produces PIs on pre-training data.}
% \tbd{I meant.. on FT data but not fine-tuned yet right? that is PIP directly after PT - just to make sure we talk about the same thing} \luo{yes.}

% 2 TDL also moves representations closer to PI space Tab \ref{tab:linear-mse-vs-pi}
% \item
% III TDL's PT probes are much better Tabs \ref{tab:linear-FT-tasks} \ref{tab:linear-dist}, \ref{tab:linear-knn}

% \maybe{IV [S] our embeddings from fine-tune data capture some homology: ask a probing model to predict [TBD D5] and show that it's considerably better on our embeddings compared to baselines, eg (we need to find a good probing task related to homology for this, and bad other embeddings; this point is not critical, but it would be very nice if we could show it) [to replace earlier \#E2, which we cannot show]
% }
% OLD TEXT
% At this point we need some verification, we have this already: showing that PIP is able to learn PIs - can predict them for FT test data after pretraining (w/o FT)... Now, below our special contributions! I'd put most focus into showing that (but I may be missing something so ideas welcome)
% Homology gives us a well-defined / reasonable embedding space to start from, due to the stability, and we just showed, that PIP can predict PIs. This is related to 2ai. I am currently still unsure how to show this. (experiments, figures, t-SNE...). maybe this is related to 2di below. we could try to compare (in any way...) any other pre-trained models embeddings w/o and combined w/ PIP?
% Homology gives us esp. a very flexible approach.
% It gives any pre-training approach or model a good initial embedding space to start from. For the former, we can maybe first pre-train with PIP and then add another method in later epochs? (currently unsure, do we need TDL for that? I don't think so...). For the latter we may experiment w/ something beyond GIN. But this only for later.



\item 
In regular class/reg experiments:
show PIP \& TDL improve (or are comparable) to:

[S] SSL SOTA Tab \ref{tab:main};

[S] real-PI+SVM or maybe better XGB [the non pre-training alternative from PIJMLR, they use SSVM]; - to show that SSL and the rest really help and PI alone is not enough \luo{Table \ref{tab:PI_method}}
% [L] rdkit+XGB or similar - copy results from moleculenet paper %[a non pre-training, common approach in the domain]


\tbd{(models) TDL+the basic ones; one additional baseline - best transformer but a recent one is also good; + JOAO?}

\tbd{(explain) pics for individual tasks on SIDER as shown on slack...} showing it's task correlation or similar that may help during FT


\item Special advantages of homology SSL

I Fig \ref{fig:small-data}\tbd{best also clintox to verify}

II Mention flexibility/potential of PIP if concatenated during FT - we have this as line in the main table
\maybe{Filtrations are very generic and can combine models during FT. a) First of all, we can say we propose this as a method to be flexible in terms of what is useful downstream. Can we show in some visual way (diagram or best, figure) that for different downstream datasets this concat approach somehow yields the best of all by guiding towards the useful ones? b)  But this also means a user can add their own, which may be even trained on different data (see below). I am currently wondering in which ways  and if this is different from combining arbitrary pre-training models. Any ideas?}

III Show how results change if we add domain-specific filtrations.

\tbd{does not have to be full table. 'just' eg 2 baselines+TDL with 2 additional filtrations} see commented parts for python package to get atom information.
%https://mendeleev.readthedocs.io/en/latest/notebooks/bulk_data_access.html - todo after install, need to downgrade two packages
% # pip install mendeleev
% OR conda install -c lmmentel mendeleev=0.13.1
% pip install pymysql==1.0.2 sqlalchemy==1.4.40
% 
% USE AS

    % attr_df =  fetch_table('elements').set_index('symbol')

    % try:
    %     mol = Chem.MolFromSmiles(smiles)
    % except:  
    %     return np.zeros(len(attr_df.columns) * 5)
    % if mol is None:
    %     return np.zeros(len(attr_df.columns) * 5)

    % atoms = [a.GetSymbol() for a in mol.GetAtoms()]
    % attrs = attr_df.loc[atoms]

III I would also show an experiment with the multi-dim filtration 

\item \maybe{I am not sure about the regression / AC data. I think it would be OK to show something just on 1 or two baselines.
for AC I don't see the experiments. the linear are good. I would do a small regression experiment on ZINC, I do not think GEOM is useful for us?
}

\item \maybe{the evaluation papers may have some interesting points which I think may make sense to consider, check these if we have time. but that's really the last point: EG 1. add 2 new lines in the table using 30 runs on (1.) scaffold and (2.) random split [to check if results are comparable]
2. [L] show that ours + concatenated rdkit (before last linear layer) is even better, and thus complementary
3.[L] does it scale with the larger pre-training data from GN22?
}


\item LIMITATIONS / OTHER POINTS 


\item FUTURE IDEAS just not to forget: 3d, PIs for augmentations, take PIs as views? expert knowledge




\end{enumerate}
